Bolocam Survey for 1.1 mm Dust Continuum Emission in the c2d Legacy Clouds. II. Ophiuchus

We present a large-scale millimeter continuum map of the Ophiuchus molecular cloud. Nearly 11 square degrees, including all of the area in the cloud with visual extinction more than 3 magnitudes, was mapped at 1.1 mm with Bolocam on the Caltech Submillimeter Observatory (CSO). By design, the map also covers the region mapped in the infrared with the Spitzer Space Telescope. We detect 44 definite sources, and a few likely sources are also seen along a filament in the eastern streamer. The map indicates that dense cores in Ophiuchus are very clustered and often found in filaments within the cloud. Most sources are round, as measured at the half power point, but elongated when measured at lower contour levels, suggesting spherical sources lying within filaments. The masses, for an assumed dust temperature of 10 K, range from 0.24 to 3.9 solar masses, with a mean value of 0.96 solar masses. The total mass in distinct cores is 42 solar masses, 0.5 to 2% of the total cloud mass, and the total mass above 4 sigma is about 80 solar masses. The mean densities in the cores are quite high, with an average of 1.6 x 10^6 per cc, suggesting short free-fall times. The core mass distribution can be fitted with a power law with slope of 2.1 plus or minus 0.3 for M>0.5 solar masses, similar to that found in other regions, but slightly shallower than that of some determinations of the local IMF. In agreement with previous studies, our survey shows that dense cores account for a very small fraction of the cloud volume and total mass. They are nearly all confined to regions with visual extinction at least 9 mag, a lower threshold than found previously.

==> table2.tex <==
\ProvidesFile{table2_new.tex}
\begin{deluxetable}{lccccccccccl}
\rotate
\tabletypesize{\scriptsize}
\tablecolumns{12}
\tablewidth{0pc}
\tablecaption{Photometry and Core Properties \label{phottab}}
\tablehead{
\colhead{ID} &  \colhead{Flux($40\arcsec$)}  &  \colhead{Flux($80\arcsec$)}  &  \colhead{Flux($120\arcsec$)} & \colhead{Total Flux}  & \colhead{Mass (10K)}  & \colhead{Peak $A_V$} & \colhead{FWHM} & \colhead{FWHM}  & \colhead{PA} & \colhead{$\mean{n}$}  & \colhead{Morphology\tablenotemark{1}} \\ 
\colhead{} &  \colhead{(Jy)}  &  \colhead{(Jy)}  &  \colhead{(Jy)} & \colhead{(Jy)}  & \colhead{($M_{\sun}$)} & \colhead{(mag)} & \colhead{(minor,$\arcsec$)} & \colhead{(major,$\arcsec$)}  & \colhead{($\degr$)}  &\colhead{cm$^{-3}$} & \colhead{}
}
\startdata
Bolo1  &  0.34 (0.03)  &   0.82 (0.07)  &   1.55 (0.1)   &  2.13 (0.13)  &  1.29 (0.08)  &  18 &  88 (0.9)  &  133 (1.4)  &  -24 (2)  &  2$\times10^5$   &  multiple,extended,round  \\
Bolo2  &  \nodata   &   \nodata   &   \nodata    &  0.46 (0.03)  &  0.28 (0.02)          &  27 &  55 (0.6)  &  58 (0.6)  &  29 (17)  &  4$\times10^5$   &  multiple,round  \\
Bolo3  &  0.46 (0.04)  &   \nodata   &   \nodata    &  0.58 (0.05)  &  0.35 (0.03)       &  22 &  53 (0.7)  &  58 (0.8)  &  88 (10)  &  5$\times10^5$   &  multiple,extended,round  \\
Bolo4  &  \nodata   &   \nodata   &   \nodata    &  0.49 (0.03)  &  0.3 (0.02)           &  28 &  52 (0.6)  &  56 (0.7)  &  -10 (11)  &  5$\times10^5$   &  multiple,elongated  \\
Bolo5  &  0.55 (0.05)  &   1.32 (0.1)  &   \nodata    &  1.61 (0.11)  &  0.97 (0.07)     &  26 &  64 (0.8)  &  70 (0.8)  &  26 (11)  &  7$\times10^5$   &  multiple,extended,elongated  \\
Bolo6  &  0.32 (0.05)  &   \nodata   &   \nodata    &  0.58 (0.08)  &  0.35 (0.05)       &  19 &  59 (1.3)  &  67 (1.5)  &  -61 (14)  &  3$\times10^5$   &  multiple,extended,weak  \\
Bolo7  &  0.56 (0.05)  &   \nodata   &   \nodata    &  1.08 (0.08)  &  0.65 (0.05)       &  29 &  56 (0.6)  &  66 (0.8)  &  -50 (6)  &  7$\times10^5$   &  multiple,extended,elongated  \\
Bolo8  &  1.86 (0.05)  &   \nodata   &   \nodata    &  3.93 (0.09)  &  2.37 (0.05)       &  98  &  55 (0.2)  &  63 (0.2)  &  81 (2)  &  3$\times10^6$   &  multiple,extended,round  \\
Bolo9  &  4.2 (0.05)  &   \nodata   &   \nodata    &  6.49 (0.08)  &  3.92 (0.05)        &  191 &  46 (0.1)  &  56 (0.1)  &  -68 (1)  &  9$\times10^6$   &  multiple,extended,round  \\
Bolo10  &  3.42 (0.05)  &   \nodata   &   \nodata    &  3.42 (0.05)  &  2.07 (0.03)      &  189 &  44 (0.1)  &  56 (0.1)  &  22 (1)  &  5$\times10^6$   &  multiple,extended,round  \\
Bolo11  &  1.72 (0.05)  &   \nodata   &   \nodata    &  1.72 (0.05)  &  1.04 (0.03)      &  88  &  49 (0.2)  &  54 (0.2)  &  50 (3)  &  2$\times10^6$   &  multiple,extended,round  \\
Bolo12  &  0.86 (0.04)  &   2.11 (0.09)  &   3.91 (0.13)   &  5.56 (0.17)  &  3.36 (0.1)  & 38  &  105 (0.5)  &  125 (0.6)  &  -45 (2)  &  4$\times10^5$   &  extended,elongated  \\
Bolo13  &  0.35 (0.04)  &   0.75 (0.08)  &   1.35 (0.12)   &  1.35 (0.12)  &  0.82 (0.07) & 16  &  76 (1.2)  &  96 (1.5)  &  44 (5)  &  2$\times10^5$   &  multiple,extended,elongated,weak  \\
Bolo14  &  0.32 (0.05)  &   0.68 (0.09)  &   1.19 (0.14)   &  1.19 (0.14)  &  0.72 (0.08) & 18  &  66 (1.2)  &  108 (2.)  &  41 (3)  &  2$\times10^5$   &  multiple,extended,weak  \\
Bolo15  &  0.61 (0.05)  &   \nodata   &   \nodata    &  0.92 (0.07)  &  0.56 (0.04)       & 31  &  50 (0.7)  &  64 (0.8)  &  19 (4)  &  8$\times10^5$   &  multiple,extended,elongated  \\
Bolo16  &  0.7 (0.05)  &   \nodata   &   \nodata    &  1.08 (0.07)  &  0.65 (0.04)        & 32  &  51 (0.6)  &  62 (0.7)  &  -58 (5)  &  9$\times10^5$   &  multiple,extended,elongated  \\
Bolo17  &  0.54 (0.05)  &   \nodata   &   \nodata    &  1.03 (0.09)  &  0.62 (0.06)        &29   &  56 (0.8)  &  68 (1.)  &  -62 (6)  &  6$\times10^5$   &  multiple,extended,elongated  \\
Bolo18  &  0.65 (0.04)  &   1.49 (0.08)  &   2.64 (0.11)   &  3.76 (0.15)  &  2.27 (0.09)  &33   &  96 (0.6)  &  149 (1.)  &  41 (1)  &  2$\times10^5$   &  extended,elongated  \\
Bolo19  &  \nodata   &   \nodata   &   \nodata    &  0.8 (0.04)  &  0.48 (0.02)            &44   &  54 (0.4)  &  58 (0.4)  &  -8 (9)  &  7$\times10^5$   &  multiple,round  \\
Bolo20  &  \nodata   &   \nodata   &   \nodata    &  0.87 (0.04)  &  0.53 (0.02)           &49   &  51 (0.4)  &  57 (0.4)  &  80 (6)  &  9$\times10^5$   &  multiple,extended,round  \\
Bolo21  &  0.82 (0.04)  &   \nodata   &   \nodata    &  1.01 (0.06)  &  0.61 (0.03)        &37   &  53 (0.5)  &  60 (0.5)  &  40 (5)  &  9$\times10^5$   &  multiple,extended,round  \\
Bolo22  &  0.77 (0.04)  &   \nodata   &   \nodata    &  0.96 (0.06)  &  0.58 (0.03)	   &35   &  54 (0.5)  &  55 (0.5)  &  -75 (61)  &  10$\times10^5$   &  multiple,extended,elongated  \\
Bolo23  &  0.55 (0.04)  &   \nodata   &   \nodata    &  0.68 (0.05)  &  0.41 (0.03)	   &28   &  53 (0.6)  &  56 (0.7)  &  -88 (20)  &  7$\times10^5$   &  multiple,extended,round  \\
Bolo24  &  0.39 (0.04)  &   \nodata   &   \nodata    &  0.39 (0.04)  &  0.24 (0.02)	   &21   &  48 (0.8)  &  57 (0.9)  &  14 (7)  &  5$\times10^5$   &  multiple,extended,elongated  \\
Bolo25  &  0.39 (0.04)  &   \nodata   &   \nodata    &  0.39 (0.04)  &  0.24 (0.02)	   &23   &  47 (0.8)  &  56 (0.9)  &  -66 (7)  &  5$\times10^5$   &  multiple,elongated  \\
Bolo26  &  0.3 (0.03)  &   0.63 (0.07)  &   1.14 (0.1)   &  1.62 (0.14)  &  0.98 (0.08)	   &16   &  108 (1.4)  &  132 (1.8)  &  84 (5)  &  9$\times10^4$   &  extended,elongated  \\
Bolo27  &  0.23 (0.03)  &   0.52 (0.07)  &   0.97 (0.1)   &  1.48 (0.13)  &  0.9 (0.08)	   &12   &  89 (1.1)  &  157 (2.)  &  58 (2)  &  9$\times10^4$   &  extended,elongated,weak  \\
Bolo28  &  0.37 (0.03)  &   0.86 (0.07)  &   1.55 (0.1)   &  2.17 (0.13)  &  1.31 (0.08)   &20   &  102 (1.)  &  113 (1.1)  &  74 (8)  &  2$\times10^5$   &  extended,elongated  \\
Bolo29  &  0.28 (0.04)  &   \nodata   &   \nodata    &  0.5 (0.07)  &  0.3 (0.04)          &20   &  54 (1.)  &  57 (1.1)  &  11 (29)  &  5$\times10^5$   &  multiple,extended,elongated  \\
Bolo30  &  0.28 (0.04)  &   \nodata   &   \nodata    &  0.46 (0.06)  &  0.28 (0.04)	   &20   &  46 (1.1)  &  57 (1.3)  &  66 (9)  &  6$\times10^5$   &  multiple,extended,elongated  \\
Bolo31  &  \nodata   &   \nodata   &   \nodata    &  0.55 (0.03)  &  0.33 (0.02)           &32   &  54 (0.5)  &  57 (0.5)  &  -61 (15)  &  5$\times10^5$   &  multiple,round  \\
Bolo32  &  \nodata   &   \nodata   &   \nodata    &  0.53 (0.03)  &  0.32 (0.02)           &31   &  56 (0.5)  &  58 (0.5)  &  74 (20)  &  4$\times10^5$   &  multiple,round  \\
Bolo33  &  0.26 (0.04)  &   0.57 (0.07)  &   \nodata    &  0.57 (0.07)  &  0.35 (0.04)	   &14   &  54 (1.2)  &  65 (1.5)  &  -33 (10)  &  4$\times10^5$   &  multiple,extended,elongated,weak  \\
Bolo34  &  0.38 (0.04)  &   0.87 (0.08)  &   \nodata    &  0.87 (0.08)  &  0.52 (0.05)	   &19   &  59 (0.9)  &  68 (1.1)  &  -73 (9)  &  4$\times10^5$   &  multiple,extended,elongated  \\
Bolo35  &  0.22 (0.04)  &   0.39 (0.08)  &   \nodata    &  0.46 (0.09)  &  0.28 (0.06)	   &13   &  66 (1.7)  &  77 (2.1)  &  40 (14)  &  2$\times10^5$   &  multiple,extended,elongated,weak  \\
Bolo36  &  1.35 (0.04)  &   \nodata   &   \nodata    &  2.49 (0.07)  &  1.51 (0.04)        &117  &  53 (0.2)  &  57 (0.2)  &  -17 (5)  &  2$\times10^6$   &  multiple,extended,round  \\
Bolo37  &  3.63 (0.04)  &   \nodata   &   \nodata    &  4.47 (0.06)  &  2.7 (0.04)         &214  &  35 (0.1)  &  45 (0.1)  &  49 (1)  &  3$\times10^7$   &  multiple,round  \\
Bolo38  &  1.52 (0.04)  &   \nodata   &   \nodata    &  2.33 (0.06)  &  1.41 (0.04)        &76   &  54 (0.2)  &  54 (0.2)  &  -15 (38)  &  2$\times10^6$   &  multiple,extended,round  \\
Bolo39  &  0.26 (0.04)  &   0.55 (0.07)  &   0.94 (0.11)   &  1.29 (0.14)  &  0.78 (0.08)  &17   &  101 (1.7)  &  128 (2.2)  &  -51 (6)  &  9$\times10^4$   &  extended  \\
Bolo40  &  1.11 (0.04)  &   \nodata   &   \nodata    &  1.67 (0.06)  &  1.01 (0.04)        &52   &  49 (0.3)  &  58 (0.3)  &  55 (3)  &  2$\times10^6$   &  multiple,extended,round  \\
Bolo41  &  0.2 (0.03)  &   0.39 (0.06)  &   0.73 (0.09)   &  0.85 (0.1)  &  0.51 (0.06)	   &11   &  40 (1.2)  &  53 (1.6)  &  -27 (9)  &  2$\times10^6$   &  multiple,extended,elongated,weak  \\
Bolo42  &  0.19 (0.03)  &   0.39 (0.07)  &   0.72 (0.1)   &  0.83 (0.11)  &  0.5 (0.07)	   &14   &  53 (1.6)  &  66 (1.9)  &  80 (11)  &  6$\times10^5$   &  multiple,extended,elongated,weak  \\
Bolo43  &  0.33 (0.04)  &   0.84 (0.07)  &   1.63 (0.11)   &  2.45 (0.15)  &  1.48 (0.09)  &20   &  98 (0.9)  &  143 (1.3)  &  47 (2)  &  1$\times10^5$   &  extended,elongated  \\
Bolo44  &  0.3 (0.03)  &   0.72 (0.06)  &   1.21 (0.09)   &  1.71 (0.12)  &  1.03 (0.08)   &15   &  96 (1.1)  &  119 (1.4)  &  55 (4)  &  1$\times10^5$   &  extended,round  \\
\cutinhead{Tentative detections in the eastern streamer}
Bolo45  &  0.20 (0.03)  &   0.47 (0.06)  &   0.94 (0.09)   &  1.36 (0.11)  &  0.82 (0.06)  &  11  &  123 (1.5)  &  157 (1.9)  &  -51 (4)  &  5$\times10^4$   &  extended,elongated,weak  \\
Bolo46  &  \nodata   &   \nodata   &   \nodata    &  0.08 (0.02)  &  0.05 (0.01)           &  7	  &  64 (3)  &  153 (6)  &  7 (3)  &  9$\times10^3$   &  extended,round,weak  \\
Bolo47  &  0.13 (0.03)  &   \nodata   &   \nodata    &  0.15 (0.04)  &  0.09 (0.02)	   &  10  &  87 (2)  &  112 (3)  &  -42 (9)  &  2$\times10^4$   &  multiple,extended,round,weak  \\
Bolo48  &  \nodata   &   \nodata   &   \nodata    &  0.86 (0.13)  &  0.52 (0.08)           &  8  &  84 (2)  &  111 (3)  &  -8 (7)  &  1$\times10^5$   &  multiple,extended,round,weak  \\
\enddata
\tablecomments{
Masses are calculated according to Equation~\ref{masseq} from the total flux density assuming a single dust temperature of $T_D=10K$ and a dust opacity at 1.1mm of $\kappa_{1.1mm} = 0.0114$~cm$^2$g$^{-1}$.  Peak $A_V$ is calculated from the peak flux density as in Equation~\ref{aveq}.  FWHM and PAs are from a Gaussian fit; the PA is measured in degrees east of north of the major axis.  $\mean{n}$ is the mean particle density as calculated from the total mass and the deconvolved average FWHM size.  Numbers in parentheses are $1\sigma$ uncertainties.  Uncertainties for masses are from photometry only, and do not include uncertainties from $\kappa$, $T_D$, or $d$, which can be up to a factor of a few or more.  Uncertainties for the FWHM and PA are formal fitting errors from the elliptical Gaussian fit; additional uncertainties of $10-15$\% apply to the FWHM, and $\sim5\degr$ to the PA (determined from simulations).}
%\tablecomments{Numbers in parentheses are $1\sigma$ uncertainties.  Masses are calculated from the total flux density assuming a single dust temperture of $T_D=10K$ and a dust opacity at 1.1mm of $\kappa_{1.1mm} = 0.0114$~cm$^2$g$^{-1}$ (see Section~\ref{masssect} for details).  FWHM and PAs are from a Gaussian fit; the PA is measured in degrees east of north of the major axis.  Mass errors are from photometry only, and do not include uncertainties from $\kappa$, $T_D$, or $d$, which can be up to a factor of a few or more.  Errors in the FWHM and PA are formal fitting errors from the elliptical Gaussian fit; additional uncertainties of $10-15$\% apply to the FWHM, adn $\sim5\degr$ to the PA (determined from simulations).}
\tablenotetext{1}{The morphology keyword(s) given indicates whether the source is multiple (within $3\arcmin$ of another source), extended (major axis FW at $2\sigma > 1\arcmin$), elongated (axis ratio at $4\sigma > 1.2$), round (axis ratio at $4\sigma < 1.2$), or weak (peak flux densities less than 8.7 times 
the RMS/beam).}
\end{deluxetable}
\endinput


==> table3.tex <==
\ProvidesFile{table3.tex}
\begin{deluxetable}{lrrrrrr}
%\rotate
%\tabletypesize{\scriptsize}
\tablecolumns{7}
\tablewidth{0pc}
\tablecaption{Cumulative Mass as a Function of Extinction \label{tab3}}
\tablehead{
\colhead{Min. $A_V$}
& \colhead{Area}
& \colhead{Cloud Mass}
& \colhead{Percent}
& \colhead{Core Mass}
& \colhead{Percent}
& \colhead{Mass Ratio\tablenotemark{1}} \\
\colhead{mag}
&  \colhead{(\%)}
&  \colhead{(\msun)}
&  \colhead{(\%)}
&  \colhead{(\msun)}
&  \colhead{(\%)}
&  \colhead{(\%)}
}
\startdata
\ 2	& 100	& 2300	& 100	& 42	& 100   & 1.8	\\
\ 4	& 39	& 1500	& 65	& 42	& 100	& 2.8	\\
\ 6	& 17	& 920	& 40	& 42	& 100	& 4.6 	\\
\ 8	& 8.8	& 640	& 28	& 39	&  93	& 6.1	\\
10	& 5.5	& 470	& 20	& 37	&  88	& 7.9 	\\
12	& 3.8	& 350	& 15	& 33	&  79	& 9.4 	\\
14	& 2.3	& 240	& 10	& 20	&  47	& 8.3 	\\
16	& 1.4	& 170	& 7.4	& 12	&  29	& 7.1 	\\
18	& 0.9	& 120	& 5.2	& 6.4	&  15	& 5.3 	\\
20	& 0.5	& \ 73	& 3.1	& 1.2	&  2.9	& 1.6	\\
\enddata
\tablecomments{
Cloud areas and masses are calculated from the extinction and conversions
from \S \ref{masssec}.  Core masses are taken from Table \ref{phottab}.
}
\tablenotetext{1}{The Mass Ratio is computed from the ratio of core mass to
cloud mass within the same contour of \av.}
\end{deluxetable}
\endinput

